Semantic Parsing of Colonoscopy Videos with Multi-Label Temporal Networks

Following the successful debut of polyp detection and characterization, more advanced automation tools are being developed for colonoscopy. The new automation tasks, such as quality metrics or report generation, require understanding of the procedure flow that includes activities, events, anatomical landmarks, etc. In this work we present a method for automatic semantic parsing of colonoscopy videos. The method uses a novel DL multi-label temporal segmentation model trained in supervised and unsupervised regimes. We evaluate the accuracy of the method on a test set of over 300 annotated colonoscopy videos, and use ablation to explore the relative importance of various method's components.

==> figures/deteced_segments.tex <==
\begin{figure*}
    % \fcapside
     \centering
    %  \hspace*{-2cm}
     \begin{subfigure}[b]{1\textwidth}
       \centering
         \includegraphics[width=\textwidth]{images/colon_seg.png}
         \caption{Video parsing output of our model.}
         \label{fig:y equals zz}
      \end{subfigure}
        
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Ileum.jpg}
         \caption{Ileum.}
         \label{fig:y equals x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Cecum.jpg}
         \caption{Cecum.}
         \label{fig:three sin x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/tools_frame.jpg}
         \caption{Tools.}
         \label{fig:five over x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/outside.jpg}
         \caption{Outside Body.}
         \label{fig:six over x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Rectum.jpg}
         \caption{Retroflextio (U-turn).}
         \label{fig:seven over x}
     \end{subfigure}
     \caption{Output of our model over a procedure together with key moments from the same video.}
     \label{fig:detected_segments}
\end{figure*}

==> figures/groupwise_mstcn.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[height=6.5cm, width=12.2cm]{images/mstcn.png} 
    \caption{Multi-Label TCN. Note that we apply the Softmax activation separately on the neurons that corresponds to the colon-segments, inside/outside and tools/no-tools.}
    \label{fig:groupwise_mstcn}
\end{figure}


==> figures/multitcn_dobule.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.7\textwidth}
   \includegraphics[height=3cm,width=1\linewidth]{images/single_tcn.png}
   \caption{}
   \label{fig:multiehad_mstcn_1} 
\end{subfigure}

\begin{subfigure}[b]{0.7\textwidth}
   \includegraphics[height=3.7cm,width=1\linewidth]{images/multistage_multihead_mstcn.png}
   \caption{}
   \label{fig:multiehad_mstcn_2}
\end{subfigure}

\caption[Two numerical solutions]{(a) Multi-Label TCN. Note that we apply the Softmax activation separately on the neurons that corresponds to the colon-segments, inside/outside and tools/no-tools. (b) Multi-Label MS-TCN with two stages.}
\label{fig:multiehad_mstcn_2}

\end{figure}

==> figures/pipeline.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[height=8cm, width=15cm]{images/op_pipeline_v2.png}
    \includegraphics[height=6.5cm, width=12.2cm]{images/pipeline.png} 
    \caption{Method overview.}
    \label{fig:pipeline}
\end{figure}

